The monodromy property for K3 surfaces allowing a triple-point-free model

The aim of this thesis is to study under which conditions $K3$ surfaces allowing a triple-point-free model satisfy the monodromy property. This property is a quantitative relation between the geometry of the degeneration of a Calabi-Yau variety $X$ and the monodromy action on the cohomology of $X$: a Calabi-Yau variety $X$ satisfies the monodromy property if poles of the motivic zeta function $Z_{X,\omega}(T)$ induce monodromy eigenvalues on the cohomology of $X$. In this thesis, we focus on $K3$ surfaces allowing a triple-point-free model, i.e., $K3$ surfaces allowing a strict normal crossings model such that three irreducible components of the special fiber never meet simultaneously. Crauder and Morrison classified these models into two main classes: so-called flowerpot degenerations and chain degenerations. This classification is very precise, which allows to use a combination of geometrical and combinatorial techniques to check the monodromy property in practice. The first main result is an explicit computation of the poles of $Z_{X,\omega}(T)$ for a $K3$ surface $X$ allowing a triple-point-free model and a volume form $\omega$ on $X$. We show that the motivic zeta function can have more than one pole. This is in contrast with previous results: so far, all Calabi-Yau varieties known to satisfy the monodromy property have a unique pole. We prove that $K3$ surfaces allowing a flowerpot degeneration satisfy the monodromy property. We also show that the monodromy property holds for $K3$ surfaces with a certain chain degeneration. We don't know whether all $K3$ surfaces with a chain degeneration satisfy the monodromy property, and we investigate what characteristics a $K3$ surface $X$ not satisfying the monodromy property should have.

==> chapters/acknowledgement/acknowledgement.tex <==
\chapter*{Dankwoord}                                  \label{ch:acknowledgement}
\addcontentsline{toc}{chapter}{Acknowledgement}
\markboth{}{}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/counterexample.tex <==
\chapter{Future research: Towards a counterexample?}\label{ch:counterexample}

Let $X$ be a $K3$ surface over $K$ with a Crauder-Morrison model that is a chain degeneration.

At the start of my PhD, we hoped that we would be able to prove that every $K3$ surface allowing a triple-point-free model satisfies the monodromy property. So far, we have not been able to do so, without limiting conditions on $X$ and we started seriously thinking about the possibility of the existence of a $K3$ surface $X$ that does \emph{not} satisfy the monodromy property. 

A $K3$ surface not satisfying the monodromy property, will be called a \emph{counterexample}. In the first section, we will look for \emph{combinatorial counterexamples}: combinatorial special fibers that, if they exist, could lead to a counterexample. So \emph{if} there exists a $K3$ surface $X$ with a Crauder-Morrison model $\X_k$ such that the special fiber $\X_k$ is a combinatorial counterexample, then the monodromy property does not hold for $X$.

In the second section, we will exclude one of the combinatorial counterexamples stated in the first section.

In Section~\ref{sect:counter-exist}, we will try to solve the existence problem: Can we construct a $K3$ surface $X$ with a model $\X$ such that the special fiber $\X_k$ is a combinatorial counterexample. This work has not been completed, but we made significant progress.

\section{Combinatorial counterexamples}


%In remark~\ref{rmk:holds-counterexample}, we already stated four combinatorial counterexamples. One of them is the following:
%
%\begin{counterexample}
%Suppose there exists a $K3$ surface $X$ over $K$ with a Crauder-Morrison model $\X$ such that the special fiber $\X_k$ has the following dual graph:
%
%\begin{center}
%\begin{tikzpicture}[scale=0.6]
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
%\node [below left] at (0,0) {$V_0$};
%\node [below right] at (0,0) {$4$};
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
%\node [below left] at (4,0) {$V_1$};
%\node [below right] at (4,0) {$2$};
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (8,0) {};
%\node [below left] at (8,0) {$V_2$};
%\node [below right] at (8,0) {$4$};
%
%
%
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,2) {};
%\node [above] at (0,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.5,2) {};
%\node [above] at (-0.5,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1,2) {};
%\node [above] at (-1,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1.5,2) {};
%\node [above] at (-1.5,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.5,2) {};
%\node [above] at (0.5,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1,2) {};
%\node [above] at (1,2) {$2$};
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1.5,2) {};
%\node [above] at (1.5,2) {$2$};
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,2) {};
%\node [above] at (4,2) {$4$};
%\node [below left] at (4,2) {$F_0$};
%
%
%\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (8,2) {};
%\node [above] at (8,2) {$8$};
%
%
%\draw (0,0) -- (4,0)
%(4,0) -- (8,0)
%(0,0) -- (0,2)
%(0,0) -- (-0.5,2)
%(0,0) -- (-1, 2)
%(0,0) -- (-1.5,2)
%(0,0) -- (0.5,2)
%(0,0) -- (1, 2)
%(0,0) -- (1.5,2)
%(4,0) -- (4,2)
%(8,0) -- (8,2)
%;
%%(0,0) -- (3,1)
%%(3,1) -- (3,2)
%%(3,2)--(3,3)
%%(3,3)--(3,4);
%\end{tikzpicture}\end{center}
%
%Suppose $V_0$ and $V_2$ are rational, ruled surfaces and $V_1$ is an elliptic ruled surface. Moreover, if we define $L_i$ as the number of blowups in the birational morphism $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$ for $i=0,1,2$, then $L_0=L_1=5$ and $L_2=1$.
%
%The seven flowers meeting $V_0$ are all of type $2A$ and the flowers meeting $V_1$ and $V_2$ are both of type $2B$.
%
%Then the monodromy property does not hold for $X$. Indeed, Theorem~\ref{thm:poles} guarantees that $-\nu_0/4$ is a pole of the motivic zeta function of $X$, where $(4, \nu_0)$ is the numerical data of $F_0$. 
%
%On the other hand, the monodromy zeta function is
%\begin{align*}
%\zeta_X(T) &= \frac{(T^4-1)^{5}}{(T^2-1)^3(T^4-1)^3(T^2-1)^7(T^4-1)(T^8-1)}\\
%&= \frac{1}{(T^2-1)^{10}(T^4+1)},
%\end{align*}
%because
%\begin{align*}
%\chi(V_0^\circ) &= 4+L_0-2\lambda_0 = -5,\\
%\chi(V_1^\circ) &= L_1-2\lambda_1 = 3,\\
%\chi(V_2^\circ) &= 4+L_2-2\lambda_2 = 3,
%\end{align*}
%where $\lambda_i$ is the number of flowers on $V_i$ for $i=0,1,2$.
%Since $\xi(F_0)=\exp(\pi i \nu_0/2)$ is not a $2$-th root of unity by Lemma~\ref{thm:holds-conic-flower-xi}, we conclude that $\xi(F_0)$ is not a monodromy eigenvalue. Therefore, $X$ does not satisfy the monodromy property.
%
%It is important to note that, a priori, we don't know whether or not a $K3$ surface with the described properties exist. Notice that at least Proposition~\ref{thm:holds-form-zeta-function-K3} is not violated.
% \qed
% \end{counterexample}

%The combinatorial counterexample 1 has index 2, but it is beneficial to study counterexamples of index 1. The reason is the following lemma.



Lemma~\ref{thm:counter-index} explains why we are mainly interested in combinatorial counterexamples of index 1: if we were able to exclude all combinatorial counterexamples of index 1, then we automatically would exclude all combinatorial counterexamples of index $2$ as well.

In order to prove that the monodromy property holds for every $K3$ surface allowing a triple-point-free model, we need to find all combinatorial counterexamples and prove that they do \emph{not} occur as special fibers of a $K3$ surface. We will exclude combinatorial counterexample~\ref{count:exclude} in Section~\ref{sect:counter-exclude}.

In order to prove that there exist a $K3$ surface with a triple-point-free model that does \emph{not} satisfy the monodromy property, we need to prove that there exists a $K3$ surface $X$ with a model $\X$ such that the special fiber is a combinatorial counterexample. In Section~\ref{sect:counter-exist}, we choose combinatorial counterexample~\ref{count:exist} and we will give some partial results regarding its existence.

%We will now give three combinatorial counterexamples of index 1. 

\begin{counterexample} \label{count:exclude}
Suppose there exists a $K3$ surface~$X$ over $K$ with a Crauder-Morrison model $\X$ such that the special fiber $\X_k$ has the following dual graph:

\begin{center}
\begin{tikzpicture}[scale=0.6]

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
\node [below left] at (0,0) {$V_0$};
\node [below right] at (0,0) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
\node [below left] at (4,0) {$V_1$};
\node [below right] at (4,0) {$2$};

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1.25,2) {};
\node [above] at (-1.25,2) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.75,2) {};
\node [above] at (-0.75,2) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.25,2) {};
\node [above] at (-0.25,2) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.25,2) {};
\node [above] at (0.25,2) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.75,2) {};
\node [above] at (0.75,2) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1.25,2) {};
\node [above] at (1.25,2) {$2$};

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (3,2) {};
\node [above] at (3,2) {$4$};
\node [below left] at (3,2) {$F_0$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (3.5,2) {};
\node [above] at (3.5,2) {$4$};

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4.5,2) {};
\node [above] at (4.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (5,2) {};
\node [above] at (5,2) {$1$};

\draw (0,0) -- (4,0)
(0,0) -- (-1.25,2)
(0,0) -- (-0.75,2)
(0,0) -- (-0.25, 2)
(0,0) -- (0.25,2)
(0,0) -- (0.75,2)
(0,0) -- (1.25,2)
(4,0) -- (3,2)
(4,0) -- (3.5, 2)
(4,0) -- (4.5, 2)
(4,0) -- (5,2);
%(0,0) -- (3,1)
%(3,1) -- (3,2)
%(3,2)--(3,3)
%(3,3)--(3,4);
\end{tikzpicture}\end{center}

Suppose $V_0$ and $V_1$ are rational, ruled surfaces. Moreover, if we define $L_i$ as the number of blowups in the birational morphism $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$ for $i=0,1$, then $L_0=6$ and $L_1=9$.

The six flowers meeting $V_0$ are all of type $2A$ and there are two flowers meeting $V_1$ of type $2A$ and two flowers of type $2B$.

Then the monodromy property does not hold for $X$. Indeed, Theorem~\ref{thm:poles} guarantees that $-\nu_0/4$ is a pole of the motivic zeta function of $X$, where $(4, \nu_0)$ is the numerical data of $F_0$. 

On the other hand, the monodromy zeta function is
\begin{align*}
\zeta_X(T) &= \frac{(T^4-1)^{2}}{(T^2-1)^5(T^2-1)^6(T^4-1)^2(T-1)^2}\\
&= \frac{1}{(T+1)^{11}(T-1)^{13}},
\end{align*}
because
\begin{align*}
\chi(V_0^\circ) &= 4+L_0-2\lambda_0 = -2,\\
\chi(V_1^\circ) &= 4+L_1-2\lambda_1 = 5,
\end{align*}
where $\lambda_i$ is the number of flowers on $V_i$ for $i=0,1$.
Since $\xi(F_0)=\exp(\pi i \nu_0/2)$ is not a $2$-th root of unity by Lemma~\ref{thm:holds-conic-flower-xi}, we conclude that $\xi(F_0)$ is not a monodromy eigenvalue. Therefore, $X$ does not satisfy the monodromy property.

It is important to note that, a priori, we don't know whether or not a $K3$ surface with the described properties exist. However, we will show in Section~\ref{sect:counter-exclude}, that there does not exist such a $K3$ surface $X$. Notice that at least Proposition~\ref{thm:holds-form-zeta-function-K3} is not violated.
 \qed
\end{counterexample}
 
\begin{counterexample} \label{count:exist}
Suppose there exists a $K3$ surface~$X$ over $K$ with a Crauder-Morrison model $\X$ such that the special fiber $\X_k$ has the following dual graph:

\begin{center}
\begin{tikzpicture}[scale=0.6]

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
\node [below left] at (0,0) {$V_0$};
\node [below right] at (0,0) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
\node [below left] at (4,0) {$V_1$};
\node [below right] at (4,0) {$1$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2.5,2) {};
\node [above] at (-2.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2,2) {};
\node [above] at (-2,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1.5,2) {};
\node [above] at (-1.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1,2) {};
\node [above] at (-1,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.5,2) {};
\node [above] at (-0.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.5,2) {};
\node [above] at (0.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1,2) {};
\node [above] at (1,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1.5,2) {};
\node [above] at (1.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2,2) {};
\node [above] at (2,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2.5,2) {};
\node [above] at (2.5,2) {$1$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,2) {};
\node [above] at (4,2) {$2$};
\node [below right] at (4,2) {$F_0$};

\draw (0,0) -- (4,0)
(0,0) -- (-2.5,2)
(0,0) -- (-2,2)
(0,0) -- (-1.5,2)
(0,0) -- (-1,2)
(0,0) -- (-0.5, 2)
(0,0) -- (0.5,2)
(0,0) -- (1,2)
(0,0) -- (1.5,2)
(0,0) -- (2,2)
(0,0) -- (2.5,2)
(4,0) -- (4,2);

\end{tikzpicture}\end{center}

Suppose $V_0$ and $V_1$ are rational, ruled surfaces. Moreover, if we define $L_i$ as the number of blowups in the birational morphism $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$ for $i=0,1$, then $L_0=10$ and $L_1=7$.

There are five flowers meeting $V_0$ of type $2A$ and five of type $2B$. The flower meeting $V_1$ is of type $2B$.

Then the monodromy property does not hold for $X$. Indeed, Theorem~\ref{thm:poles} guarantees that $-\nu_0/2$ is a pole of the motivic zeta function of $X$, where $(2, \nu_0)$ is the numerical data of $F_0$. 

On the other hand, the monodromy zeta function is
\begin{align*}
\zeta_X(T) &= \frac{(T^2-1)^{6}}{(T-1)^9(T^4-1)^5(T-1)^5(T^2-1)}\\
&= \frac{1}{(T^2+1)^{5}(T-1)^{14}},
\end{align*}
because
\begin{align*}
\chi(V_0^\circ) &= 4+L_0-2\lambda_0 = -6,\\
\chi(V_1^\circ) &= 4+L_1-2\lambda_1 = 9,
\end{align*}
where $\lambda_i$ is the number of flowers on $V_i$ for $i=0,1$.
Since $\xi(F_0)=\exp(\pi i \nu_0)\neq 1$, by Lemma~\ref{thm:holds-conic-flower-xi}, we conclude that $\xi(F_0)$ is not a monodromy eigenvalue. Therefore, $X$ does not satisfy the monodromy property.

It is important to note that, a priori, we don't know whether or not a $K3$ surface with the described properties exist. In Section~\ref{sect:counter-exist}, we will give some partial results regarding the existence of such a $K3$ surface $X$. Notice that at least Proposition~\ref{thm:holds-form-zeta-function-K3} is not violated.
 \qed
\end{counterexample}

The following combinatorial counterexample has a chain where only one end component is a rational, ruled surface. 

\begin{counterexample}
Suppose there exists a $K3$ surface~$X$ over $K$ with a Crauder-Morrison model $\X$ such that the special fiber $\X_k$ has the following dual graph:

\begin{center}
\begin{tikzpicture}[scale=0.6]

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
\node [below left] at (0,0) {$V_0$};
\node [below right] at (0,0) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
\node [below left] at (4,0) {$V_1$};
\node [below right] at (4,0) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (8,0) {};
\node [below left] at (8,0) {$V_2$};
\node [below right] at (8,0) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (12,0) {};
\node [below left] at (12,0) {$V_3$};
\node [below right] at (12,0) {$3$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2.5,2) {};
\node [above] at (-2.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2,2) {};
\node [above] at (-2,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1.5,2) {};
\node [above] at (-1.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1,2) {};
\node [above] at (-1,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.5,2) {};
\node [above] at (-0.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.5,2) {};
\node [above] at (0.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1,2) {};
\node [above] at (1,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1.5,2) {};
\node [above] at (1.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2,2) {};
\node [above] at (2,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2.5,2) {};
\node [above] at (2.5,2) {$1$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,2) {};
\node [above] at (4,2) {$2$};
\node [below right] at (4,2) {$F_0$};

\draw (0,0) -- (4,0)
(0,0) -- (-2.5,2)
(0,0) -- (-2,2)
(0,0) -- (-1.5,2)
(0,0) -- (-1,2)
(0,0) -- (-0.5, 2)
(0,0) -- (0.5,2)
(0,0) -- (1,2)
(0,0) -- (1.5,2)
(0,0) -- (2,2)
(0,0) -- (2.5,2)
(4,0) -- (4,2)
(4,0)--(8,0)
(8,0)--(12,0);

\end{tikzpicture}\end{center}

Suppose $V_0$ is a rational, ruled surfaces, $V_1$ and $V_2$ are elliptic ruled surfaces and $V_3\simeq \P^2$. Moreover, if we define $L_i$ as the number of blowups in the birational morphism $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$ for $i=0,1, 2$, then $L_0=10$ and $L_1=2$ and $L_2=0$.

There are five flowers meeting $V_0$ of type $2A$ and five of type $2B$. The flower meeting $V_1$ is of type $2B$.

Then the monodromy property does not hold for $X$. Indeed, Theorem~\ref{thm:poles} guarantees that $-\nu_0/2$ is a pole of the motivic zeta function of $X$, where $(2, \nu_0)$ is the numerical data of $F_0$. 

On the other hand, the monodromy zeta function is
\begin{align*}
\zeta_X(T) &= \frac{(T^2-1)^{6}}{(T^3-1)^3(T^4-1)^5(T-1)^5(T^2-1)}\\
&= \frac{1}{(T^3-1)^3(T^2+1)^{5}(T-1)^{5}},
\end{align*}
because
\begin{align*}
\chi(V_0^\circ) &= 4+L_0-2\lambda_0 = -6,\\
\chi(V_1^\circ) &= L_1-2\lambda_1 = 0,\\
\chi(V_2^\circ) &= L_2-2\lambda_2 = 0,\\
\chi(V_3^\circ) &= 3-2\lambda_3 = 3,
\end{align*}
where $\lambda_i$ is the number of flowers on $V_i$ for $i=0,1,2,3$.
Since $\xi(F_0)=\exp(\pi i \nu_0)\neq 1$, by Lemma~\ref{thm:holds-conic-flower-xi}, we conclude that $\xi(F_0)$ is not a monodromy eigenvalue. Therefore, $X$ does not satisfy the monodromy property.

It is important to note that, a priori, we don't know whether or not a $K3$ surface with the described properties exist. Notice that at least Proposition~\ref{thm:holds-form-zeta-function-K3} is not violated.
 \qed
 \end{counterexample}
 
 \subsubsection*{How to find combinatorial counterexamples?}
Combinatorial counterexamples can be constructed using similar techniques as in the proof of Theorem~\ref{thm:holds-chain-extra}. We will explain this briefly for combinatorial counterexamples with the following chain:

\begin{center}
\begin{tikzpicture}[scale=0.6]

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
\node [below left] at (0,0) {$V_0$};
\node [below right] at (0,0) {$2N$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
\node [below left] at (4,0) {$V_1$};
\node [below right] at (4,0) {$N$};

\draw (0,0) -- (4,0);

\end{tikzpicture}\end{center}
So suppose there exist a $K3$ surface $X$ of index $\iota(X)=1$ with a Crauder-Morrison model $\X$. Suppose $\X$ is a chain degeneration with chain as above and assume that both $V_0$ and $V_1$ are rational, ruled surfaces. Assume moreover, that $X$ does not satisfy the monodromy property.

Let $\phi$ be the total number of flowers of type $2B$ and $2C$ meeting $V_1$ and let $\gamma$ be the total number of flowers of type $2A$ meeting $V_1$. Moreover, let $\phi'$ be the total number of flowers of type $2B$ and $2C$ meeting $V_0$ and let $\gamma'$ be the total number of flowers of type $2A$ meeting $V_0$.

Because of Lemma~\ref{thm:CM-euler-characteristics}, the monodromy zeta function is given by
\begin{equation}
\zeta_X(T) = \frac{(T^{2N} - 1)^{- \chi(V_0^{\circ})}}{(T^{N} - 1)^{\chi(V_1^{\circ})} (T^{4N} - 1)^{\phi'}(T^{N} - 1)^{\gamma'} (T^{2N} - 1)^{\phi}(T^{N/2} - 1)^{\gamma} }. \label{eq:zetafunction'}
\end{equation}

Because $X$ has index $\iota(X)=1$, by Proposition~\ref{thm:holds-index}, this means that $\gcd_{i\in I} N_i = 1$. Therefore
\begin{equation}
N = \begin{cases}
1 & \text{if } \gamma=0,\\
2 & \text{if } \gamma>0.\\
\end{cases} \label{eq:index'}
\end{equation}

For $i=0,1$, let $L_i$ be the number of blowups in the contraction $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$.

Lemma~\ref{thm:hold-relation-L} implies that 
\begin{equation}
L_0+2 L_1 = 24.
\end{equation}
In particular, 
\begin{equation}L_0 \text{ is even}.\end{equation}


From Lemma~\ref{thm:holds-relation-L-flower}, it follows that 
\begin{equation}
\phi'+\gamma'-L_0 \leq 2, 
\end{equation}

and

\begin{equation}
\phi+\gamma-L_1 \leq 2.
\end{equation}

Define $I^\dagger\subset I$ to be the set of indices $i\in I$ where either
$\rho_i$ is minimal, or
$E_i$ is the top of a conic-flower.
Let $S^\dagger=\{(-\nu_i,N_i)\in \Z\times \Z_{>0}\mid i\in I^\dagger\}$. Corollary~\ref{thm:poles-contributions} says that
\[Z_{X,\omega}^{\hat{\mu}}(T)\in \mathcal{M}_k^{\hat{\mu}}\left[T, \frac{1}{1-\L^{a}T^b}\right]_{(a,b)\in S^\dagger}.\]
By Theorem~\ref{thm:holds-lct}, we know that $\xi(E_i)$ is a monodromy eigenvalue if $\rho_i$ is minimal. Therefore, there must be a conic-flower $F$ such that $\xi(F_0)$ is \emph{not} a monodromy eigenvalue. By Proposition~\ref{thm:CM-chain-flowers}, the flower $F$ is of type $2B$ or $2C$.

Suppose $F$ meets $V_0$. Then $N(F_0)=4N$, and by Lemma~\ref{thm:holds-conic-flower-xi}, we have that $\xi(F_0)$ is not a $2N$-th root of unity. Therefore $\xi(F_0)$ is a monodromy eigenvalue, contrary to our assumption.

This means that $F$ meets $V_1$ and $N(F_0)=2N$. By definition of $\phi$, we have 
\begin{equation}\phi\geq 1. \end{equation}
By Lemma~\ref{thm:holds-conic-flower-xi}, we have that $\xi(F_0)$ is not a $N$-th root of unity, and therefore we must have
$-\chi(V_0^\circ) = \phi+\phi'$.

%We have
%\[
%\chi(V_i) = \begin{cases}
%L_i & \text{for } i \in \{ 1, \ldots, k\},\\
%4+L_i & \text{for } i \in \{0, k+1 \}.
%\end{cases}
%\]

We have $\chi(V_0^{\circ}) = 4 + L_0 -2\phi' - 2\gamma'$.
Therefore
\begin{equation}\phi'+2\gamma'-\phi-L_0 = 4,
\end{equation}
and equation~\eqref{eq:zetafunction'} can be written as
\begin{equation*}
\zeta_X(T) = \frac{1}{(T^{N} - 1)^{\chi(V_1^{\circ})} (T^{2N} + 1)^{\phi'}(T^{N} - 1)^{\gamma'} (T^{N/2} - 1)^{\gamma} }. 
\end{equation*}
Proposition~\ref{thm:holds-form-zeta-function-K3} gives that
\[\chi(V_1^{\circ}) + 2\phi'+\gamma'+ \frac{\gamma}{2}=\frac{24}{N}. \]

Since $\chi(V_1^\circ)=4+L_1-2\phi-2\gamma$, we get
\begin{equation}
L_1+2\phi'+\gamma' -2\phi - \frac{3\gamma}{2} = \frac{24}{N} - 4. \label{eq:geen-inspiratie}
\end{equation}

So therefore, finding combinatorial counterexamples with a chain $2NV_0+NV_1$ where $V_0$ and $V_1$ are rational, ruled surfaces comes down to finding integer solutions for $N, \phi, \gamma, \phi', \gamma', L_0, L_1$ satisfying equations \eqref{eq:index'} -- \eqref{eq:geen-inspiratie}.




\section{Excluding a combinatorial counterexample} \label{sect:counter-exclude}

In this section we will prove that there does not exist a $K3$ surface $X$ with a model $\X$ such that the special fiber $\X_k$ satisfies the description of combinatorial counterexample~\ref{count:exclude}. So suppose there exists such a $K3$ surface $X$.

Denote by $C_1=V_0\cap V_1$ and $C_2, \ldots, C_7$ the flowercurves on $V_0$. We know that $C_1$ is an elliptic curve and $C_2, \ldots, C_7$ are rational curves. Moreover, they are pairwise disjoint as there are no triple points.

Let $\Y$ be the normalization of $\X\times_R R[\pi]/(\pi^4-t)$.
Proposition \ref{thm:poles-local-comp-etale-branch} gives that $f_ {V_0}$ is \'etale above $V_0^\circ$ of degree 4 and that it is ramified of index 2 above $C_1, \ldots, C_7$. 
Therefore, $\Y\to \X$ is an $n$-cyclic cover, with $n=2$ or $4$.

In \cite[Section I.17]{BHPV}, it is explained that the existence of this $n$-cyclic cover implies the existence of a line bundle $\mathcal{L}$ with
\[\mathcal{L}^{\otimes n} = \O_{V_0}(C_1+C_2+\cdots + C_7).\]

Let $D$ be the divisor associated with the line bundle $\mathcal{L}$. We certainly have $nD \equiv C_1+C_2+\cdots+ C_7$, and therefore, we find
\begin{align*}
n^2 D^2 &= 	(C_1+C_2+\cdots + C_7)^2\\
	&=		 (C_1^2+C_2^2+\cdots +C_7^2),
\end{align*}
where we used in the second equality that $C_1, \cdots , C_7$ are pairwise disjoint.
From Lemma~\ref{thm:CM-self-intersection-flower-curve}, we know that $C_2^2=\cdots = C_7^2=-2$. Moreover, from equation~\eqref{eq:canonical-bundle-component-general} and Remark~\ref{rmk:CM-canonical-bundle-min-weight}, it follows that
\[K_{V_0}\equiv C_1.\]
Hence, because $L_0=6$, we have $C_1^2= 2$, by \cite[Corollary~V.2.11 and Proposition~V.3.3]{Hartshorne} 


We conclude that $n^2D^2=10$ and hence $D^2$ is not an integer. As a consequence, an $n$-cyclic cover of $V_0$ ramified along $C_1+\cdots + C_7$ does not exist. 
We conclude that there does not exist a $K3$ surface $X$ with the described properties.

%Denote $\mathcal{E}=V_1\cap V_2$. By subsection \ref{subsec:V_2}, we know that $f^{-1}(\mathcal{E})\to \mathcal{E}$ is non ramified of degree 2. This means that $f^{-1}(\mathcal{E})$ is either connected or contains two components. By the Hurwitz formula, the components of $f^{-1}(\mathcal{E})$ are elliptic.
%
%If $f^{-1}(\mathcal{E})$ is connected, then $f^{-1}(V_1)$ must also be connected and meets 12 flowers.
%
%If $f^{-1}(\mathcal{E})$ has two components, then $f^{-1}(V_1)$ must also contain two components and each component meets 6 flowers. (Galois action and subsection \ref{subsec:FlowerV_1}).




\section{Existence of a counterexample} \label{sect:counter-exist}

The aim of this section is to prove that there exists a $K3$ surface $X$ over $K$ with a model $\X$ such that the special fiber $\X_k$ is described by combinatorial counterexample~\ref{count:exist}. This work has not been finished. In the first subsection, we explain the strategy. In the next five sections, important steps are worked out. In the final section, we explain the work that still needs to be done to find a $K3$ surface not satisfying the monodromy property.

Let's recall the details of combinatorial counterexample~\ref{count:exist}.
We will try to prove that there exists a $K3$ surface~$X$ over $K$ with a Crauder-Morrison model $\X$ such that the special fiber $\X_k$ has the following dual graph:

\begin{center}
\begin{tikzpicture}[scale=0.6]

\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0,0) {};
\node [below left] at (0,0) {$V_0$};
\node [below right] at (0,0) {$2$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,0) {};
\node [below left] at (4,0) {$V_1$};
\node [below right] at (4,0) {$1$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2.5,2) {};
\node [above] at (-2.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-2,2) {};
\node [above] at (-2,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1.5,2) {};
\node [above] at (-1.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-1,2) {};
\node [above] at (-1,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (-0.5,2) {};
\node [above] at (-0.5,2) {$4$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (0.5,2) {};
\node [above] at (0.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1,2) {};
\node [above] at (1,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (1.5,2) {};
\node [above] at (1.5,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2,2) {};
\node [above] at (2,2) {$1$};
\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (2.5,2) {};
\node [above] at (2.5,2) {$1$};


\node [draw,shape=circle, fill, inner sep=0pt,minimum size=3pt] at (4,2) {};
\node [above] at (4,2) {$2$};
\node [below right] at (4,2) {$F_0$};

\draw (0,0) -- (4,0)
(0,0) -- (-2.5,2)
(0,0) -- (-2,2)
(0,0) -- (-1.5,2)
(0,0) -- (-1,2)
(0,0) -- (-0.5, 2)
(0,0) -- (0.5,2)
(0,0) -- (1,2)
(0,0) -- (1.5,2)
(0,0) -- (2,2)
(0,0) -- (2.5,2)
(4,0) -- (4,2);

\end{tikzpicture}\end{center}

The surfaces $V_0$ and $V_1$ are rational, ruled. If we define $L_i$ to be the number of blowups in the birational morphism $V_i\to \overline{V}_i$ to the minimal ruled surface $\overline{V}_i$ for $i=0,1$, then $L_0=10$ and $L_1=7$.

There are five flowers meeting $V_0$ of type $2A$ and five of type $2B$. The flower meeting $V_1$ is of type $2B$.

It is explained in combinatorial counterexample~\ref{count:exist}, that if such a $K3$ surface $X$ existed, then it would not satisfy the monodromy property.

\subsection{Strategy}

\textbf{Step 1.} We need to check that all components described in combinatorial counterexample~\ref{count:exist} indeed exist. We also need to check that on each component, the desired double curves exist.

\textbf{Step 2.}
Suppose there exists a $K3$ surface $X$ over $K$ with an $snc$-model $\X$ such that the special fiber $\X_k$ is as described above. By the semi-stable reduction theorem, there exists a finite extension $L$ of $K$ such that $X\times_K L$ has a Kulikov model $\Y$ as in Theorem~\ref{thm:pre-Kulikov}. It is possible to compute $\Y_k$ explicitly.

\textbf{Step 3.}
We need to prove that $\Y_k$, as computed in step 1, is a $d$-semi-stable $K3$ surface. A result by Friedman in \cite{Friedman}, asserts that there exists a $K3$ surface $Y$ over $L$ with an $snc$-model $\Y$ such that the special fiber $\Y_k$ is indeed as computed in step 1.

\textbf{Step 4.} 
Denote by $G=\Gal(L/K)$. There is a natural $G$-action on every component of $\Y_k$. \todo{This is false. Give correction.} We need to check that such a $G$-action indeed exists on every component of $\Y_k$.

\textbf{Step 5.}
The result of Friedman needs to be generalized such that the action on $\Y_k$ can be lifted to $\Y$. \todo{This is false.}

\textbf{Step 6.}
Let $\widetilde{\X}$ be the quotient scheme $\Y/G$. \todo{Not $\Y/G$.} Its general fiber is a $K3$ surface $X$ over $K$. We need to prove that, by contracting components in $\widetilde{\X}_k$, we get a Crauder-Morrison model $\X$, such that the special fiber $\X_k$ equals the combinatorial counterexample~\ref{count:exist}. Therefore, $X$ does not satisfy the monodromy property.

In Section~\ref{sect:count-existence}, we work out the details of step 1. We compute $\Y_k$ as described in step 2, in sections \ref{sect:count-base-change}, \ref{sect:count-desing} and \ref{sect:count-Kulikov}. In Section~\ref{sect:count-Friedman}, we prove the claim in step 3. 
Steps 4, 5 and 6 are not done in this thesis, and we hope that someone will carry them out in the future. 



%\subsection{Existence of the components} \label{sect:count-existence}
%
%\subsubsection{Components of the flowers}
%
%Let $F$ be a component of a flower in combinatorial counterexample~\ref{count:exist}. Then $F\simeq \P^2$ and the double curve is either a line or a conic. Such a component certainly exists.
%
%\subsubsection{The component $V_1$}
%
%The component $V_1$ should be a rational, ruled surface with $L_1=7$. It should allow an elliptic curve $C_1$ with $K_{V_1}\equiv -C_1$, and a rational curve $C_2$ with $C_2^2=-2$. Moreover, $C_1$ and $C_2$ should be disjoint. 
%
%%Let $V_1\to\overline{V}_1$ be the contraction of $V_1$ to the minimal ruled surface $\overline{V}_1$. Define $e$ such that $\overline{V}_1=\Sigma_e$, the $e$-th Hirzebruch surface. As in the proof of Proposition~\ref{thm:CM-chain-structure-fibers}, we know that $K_{\overline{V}_1}\equiv \overline{C}_1$. 
%%Therefore, by \cite[Corollary~V.2.11]{Hartshorne}, we have $\overline{C}_1\equiv 2D+(2+e)\fiber$, where $D$ is the section on $\overline{V}_1$ with $\O_{\overline{V}_1}(\overline{C}_1) = \O_{\overline{V}_1}(1)$, and where $\fiber$ is a general fiber of the ruling on $\overline{V}_1$. We conclude that $e\in \{0,1,2\}$, by \cite[Proposition~V.2.20]{Hartshorne}.
%
%Set $\overline{V}_1=\Sigma_2$, the $2$-nd Hirzebruch surface. Let $\overline{C}_2$ be the unique section on $\overline{V}_1$ with $\overline{C}_2^2=-2$ and let $\fiber$ be a general fiber of the ruling on $\overline{V}_1$. By \cite[Corollary~V.2.11]{Hartshorne}, we have that $K_{\overline{V}_1}\equiv -2\overline{C}_2 - 4\fiber$ and \cite[Proposition~V.2.18]{Hartshorne} guarantees that there is a smooth, irreducible curve $\overline{C}_1$ with $K_{\overline{V}_1}\equiv - \overline{C}_1$.
%We can compute that $\overline{C}_2$ and $\overline{C}_1$ are disjoint.
%
% Let $V_1$ be the surface obtained from $\overline{V}_1$ by blowing up seven points on $\overline{C}_1$. Let $C_1$ and $C_2$ be the strict transforms of $\overline{C}_1$ and $\overline{C}_2$ respectively. We then have that $C_2$ is a rational curve with $C_2^2=-2$, disjoint from $C_1$.
% By \cite[Proposition~3.3]{Hartshorne} and \cite[Proposition~3.6]{Hartshorne}, we know that $K_{V_1}\equiv -C_1$. Lemma~\ref{thm:CM-chain-exceptional-curve} gives that $C_1$ is an elliptic curve.
% 
%\subsubsection{The component $V_0$}
%
%The component $V_0$ should be a rational, ruled surface with $L_0=10$. It should allow an elliptic curve $C_1$ with $K_{V_0}\equiv -C_1$, and ten rational curves $C_2, \ldots, C_{11}$ with $C_i^2=-2$, for every $i=2,\ldots, 11$. Moreover, $C_1, C_2, \ldots, C_{11}$ should be pairwise disjoint.
%
%Let $\overline{V}_0=\Sigma_1$, the $1$-st Hirzebruch surface, i.e.,  $\overline{V}_0$ is isomorphic to $\P^2$ blown up in one point. Let $\overline{C_2}$ be the unique section with $\overline{C}_2^2=-1$ and let $\fiber$ be a general fiber of the ruling on $\overline{V}_0$. 
%By \cite[Corollary~V.2.11]{Hartshorne}, we have that $K_{\overline{V}_1}\equiv -2\overline{C}_2 - 3\fiber$ and \cite[Proposition~V.2.18]{Hartshorne} guarantees that there is a smooth, irreducible curve $\overline{C}_1$ with $K_{\overline{V}_1}\equiv - \overline{C}_1$.
%We can compute that $\overline{C}_2$ and $\overline{C}_1$ are disjoint. Let $\widetilde{\fiber}$ to be the fiber through $\overline{C}_1\cap \overline{C}_2$.
%
%Consider four sections $\overline{C}_3, \overline{C}_4, \overline{C}_5, \overline{C}_6$ on $\overline{V}_0$, all numerically equivalent to $\overline{C}_2+\fiber$, with $\bigcap_{i=3}^6 \overline{C}_i=\{P\}$, where $P$ is a point on $\overline{C}_1\cap \widetilde{\fiber}$ . \question{Should I say something about why that exists?} Moreover, we can compute that $\overline{C}_2\cdot \overline{C}_i=0$ and $\overline{C}_i^2=1$ for $i=3,\ldots, 6$.
%\note{
%This exists. Suppose $\overline{V}_0$ is $\P^2$ blown up in a point on $\overline{C}_1$. Without loss of generality, we can assume that point is $(0,0,1)$. Consider a point that lies on the line through $(0,0,1)$ tangent to $\overline{C}_1$. Without loss of generality, we can assume this point is $(1,0,0)$. In $\P^2$, consider four lines that intersect each other in $(1,0,0)$ and that are disjoint from $(0,0,1)$. (By writing down explicit equations, we can find such lines: the lines $(1,0,0) -- (0,1,0)$, $(1,0,0)--(1,1,0)$, $(1,0,0)--(1,2,0)$ and $(1,0,0)--(2,1,0)$.) Then we have that every one of these four lines, after blowing up, is disjoint with the exceptional divisor $\overline{C}_2$. Moreover, let $L$ be the strict transform of one of these lines. We can write $L\equiv a\overline{C}_2+b\fiber$. Since the blow up is an isomorphism away from the point in which we blew up, we have $L^2=1$, and therefore $a(2b-a)=1$. Since $L$ and $\overline{C}_2$ are disjoint, we have $-a+b=0$. We conclude that $a^2=1$ and $b=a$. Because of \cite[V.2.18]{Hartshorne}, we conclude $a=1$.
%} 
%
%Let $V^{(9)}$ be the blowup of $V^{(10)}=\overline{V}_0$ in the point $P$. Let $C_i^{(9)}$ be the strict transforms of $\overline{C}_i$ for $i=1, \ldots, 6$. We then have that $C_2^{(9)}, \ldots, C_6^{(9)}$ are pairwise disjoint.
%Moreover, $\left(C_i^{(9)}\right)^2=0$ for $i=3,\ldots, 6$. The ruled surface $V^{(9)}$ has one irreducible fiber. A sketch can be found in figure~\ref{fig:count-V^9}. We see the five sections. The dotted lines are (components of) fibers of the ruling. The labels are the self-intersections of the curves.
%
%\begin{figure}[H]
%
%\minipage{0.5\textwidth}
%\begin{tikzpicture}[scale = 0.4]
%\draw[dashed] (-4,4) -- (4,4);
%\draw[dashed] (-4,1.5) -- (4,1.5);
%\draw[dashed] (-4,0.5)--(4,0.5);
%\draw[dashed] (-4,-0.5) -- (4,-0.5);
%\draw[dashed] (-4,-1.5) -- (4,-1.5);
%
%\draw (-0.5,4.5) -- (0.6,2.25);
%\draw (0.6,2.75) -- (-0.5,-2);
%
%\node[right] at (4,4) {\small{$-1$}};
%\node[right] at (4,1.5) {\small{$0$}};
%\node[right] at (4,0.5) {\small{$0$}};
%\node[right] at (4,-1.5) {\small{$0$}};
%\node[right] at (4,-0.5) {\small{$0$}};
%
%\node[left] at (-4,4) {\small{$C_2^{(9)}$}};
%\node[left] at (-4,1.5) {\small{$C_3^{(9)}$}};
%\node[left] at (-4,0.5) {\small{$C_4^{(9)}$}};
%\node[left] at (-4,-1.5) {\small{$C_6^{(9)}$}};
%\node[left] at (-4,-0.5) {\small{$C_5^{(9)}$}};
%
%\node[above] at (-0.5,4.5) {\small{$-1$}};
%\node[below] at (-0.5,-2) {\small{$-1$}};
%
%\node[] at (7, 0) {$\longrightarrow$};
%
%%\node [shape=circle, fill, inner sep=0pt,minimum size=4pt] at (-0.4,4) {};
%\end{tikzpicture}
%\endminipage\hfill%
%%
%\minipage{0.5\textwidth}
%\centering
%\begin{tikzpicture}[scale = 0.4]
%\draw[dashed] (-4,4) -- (4,4);
%
%\draw (0,4.5) -- (0,-1.5);
%
%\draw [dashed] plot [smooth] coordinates {(-4,1.5) (-2,1) (0,0) (2,-1) (4,-1.5)};
%\draw [dashed] plot [smooth] coordinates {(-4,-1.5) (-2,-1) (0,0) (2,1) (4,1.5)};
%\draw [dashed] plot [smooth] coordinates {(-4,0.5) (-2,0.25) (0,0) (2,-0.25) (4,-0.5)};
%\draw [dashed] plot [smooth] coordinates {(-4,-0.5) (-2,-0.25) (0,0) (2,0.25) (4,0.5)};
%
%\node[right] at (4,4) {\small{$-1$}};
%\node[right] at (4,1.5) {\small{$1$}};
%\node[right] at (4,0.5) {\small{$1$}};
%\node[right] at (4,-1.5) {\small{$1$}};
%\node[right] at (4,-0.5) {\small{$1$}};
%
%\node[left] at (-4,4) {\small{$C_2^{(10)}$}};
%\node[left] at (-4,1.5) {\small{$C_3^{(10)}$}};
%\node[left] at (-4,0.5) {\small{$C_4^{(10)}$}};
%\node[left] at (-4,-1.5) {\small{$C_6^{(10)}$}};
%\node[left] at (-4,-0.5) {\small{$C_5^{(10)}$}};
%
%\node[above] at (0,4.5) {\small{$0$}};
%\node[below] at (0,-1.5) {\small{$\widetilde{\fiber}$}};
%
%\node [shape=circle, fill, inner sep=0pt,minimum size=4pt] at (0,0) {};
%\end{tikzpicture}
%\endminipage \hfill
%%
%\caption{$V^{(9)}\to V^{(10)}$}
%\label{fig:count-V^9}
%\end{figure}
%
%Let $V^{(8)}$ be the blow-up of $V^{(9)}$ in $C_1^{(9)}\cap C_2^{(9)}$. By the choice of $\fiber$ an the fact that $P\in \overline{C}_1\cap \fiber$, the center of blowing up, is a point on the unique reducible fiber. Let $\fiber_1^{(8)}, \fiber_2^{(8)}$ and $\fiber_3^{(8)}$ be the components of the reducible fiber as seen in the sketch of figure~\ref{fig:count-V^8}
%
%\begin{figure}[H]
%
%\minipage{0.5\textwidth}
%\begin{tikzpicture}[scale = 0.4]
%\draw [dashed] (-4,4) -- (4,4);
%\draw [dashed] (-4,0.25)--(4,0.25);
%\draw [dashed] (-4,-0.25) -- (4,-0.25);
%\draw [dashed] (-4,-0.75) -- (4,-0.75);
%\draw [dashed] (-4,-1.25) -- (4,-1.25);
%
%\draw (-0.5,4.5) -- (0.6,2.5);
%\draw (0.6,1.5) -- (-0.7,-2);
%\draw (0.4, 3.5) -- (0.4, 0.5);
%
%\node[right] at (4,4) {\small{$-2$}};
%%\node[right] at (4,1.5) {\small{$0$}};
%%\node[right] at (4,0.5) {\small{$0$}};
%\node[right] at (4,-0.5) {\small{$0$}};
%%\node[right] at (4,-0.5) {\small{$0$}};
%
%
%\node[above] at (-0.5,4.5) {\small{$\fiber_1^{(8)}$}};
%\node[below] at (-0.5,-2) {\small{$\fiber_3^{(8)}$}};
%\node[right] at (0.4, 3.5) {\small{$\fiber_2^{(8)}$}};
%
%
%\node[] at (7, 0) {$\longrightarrow$};
%
%%\node [shape=circle, fill, inner sep=0pt,minimum size=4pt] at (-0.4,4) {};
%\end{tikzpicture}
%\endminipage\hfill%
%%
%\minipage{0.5\textwidth}
%\centering
%\begin{tikzpicture}[scale = 0.4]
%\draw [dashed](-4,4) -- (4,4);
%\draw [dashed](-4,0.25)--(4,0.25);
%\draw [dashed](-4,-0.25) -- (4,-0.25);
%\draw [dashed](-4,-0.75) -- (4,-0.75);
%\draw [dashed](-4,-1.25) -- (4,-1.25);
%
%\draw (-0.5,4.5) -- (0.6,2.25);
%\draw (0.6,2.75) -- (-0.5,-2);
%
%\node[right] at (4,4) {\small{$-1$}};
%%\node[right] at (4,1.5) {\small{$0$}};
%%\node[right] at (4,0.5) {\small{$0$}};
%\node[right] at (4,-0.5) {\small{$0$}};
%%\node[right] at (4,-0.5) {\small{$0$}};
%
%
%\node[above] at (-0.5,4.5) {\small{$-1$}};
%\node[below] at (-0.5,-2) {\small{$-1$}};
%
%
%\node [shape=circle, fill, inner sep=0pt,minimum size=4pt] at (-0.25555,4) {};
%\end{tikzpicture}
%\endminipage \hfill
%%
%\caption{$V^{(8)}\to V^{(9)}$}
%\label{fig:count-V^8}
%\end{figure}
%
%We have $\left(\fiber_1^{(8)}\right)^2=\left(\fiber_3^{(8)}\right)^2=-1$ and $\left(\fiber_2^{(8)}\right)^2=-2$. Moreover, it can be computed that 
%\[K_{V^{(8)}}\equiv -2C_2^{(8)}-3\fiber - \fiber_1^{(8)}+\fiber_3^{(8)},\]
%where $\fiber$ is a general fiber of the ruling on $V^{(8)}$.
%
%\note{ 
%\[K_{V^{(9)}}\equiv \pi^*K_{V^{(10)}} + \fiber_3^{(9)} \equiv -2C_2-3\fiber + \fiber_3.\]
%Therefore
%\[K_{V^{(8)}}\equiv -2C_2^{(8)}-2\fiber_1-3\fiber +\fiber_3^{(8)}+ \fiber_1^{(8)}\]
%}
%
%\subsection{Base change and normalization} \label{sect:count-base-change}
%
%\subsection{Desingularization} \label{sect:count-desing}
%
%\subsection{Contractions to the Kulikov model} \label{sect:count-Kulikov}
%
%\subsection{Existence of ...} \label{sect:count-Friedman}
%\todo{Find title}



\section{Open questions}
Obviously: does this counterexample exist?

If yes: Does this have an influence on the monodromy conjecture for hypersurface singularities?

If yes: Can we characterize the extra poles? What do we know about them? Where do they come from? 

If no: Complete the proof for chain degenerations. More general: for $K3$ surfaces. Even more general: for Calabi-Yau varieties.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}

